Dynamic Sub-Cluster-Aware Network for Few-Shot Skin Disease Classification

This paper addresses the problem of few-shot skin disease classification by introducing a novel approach called the Sub-Cluster-Aware Network (SCAN) that enhances accuracy in diagnosing rare skin diseases. The key insight motivating the design of SCAN is the observation that skin disease images within a class often exhibit multiple sub-clusters, characterized by distinct variations in appearance. To improve the performance of few-shot learning, we focus on learning a high-quality feature encoder that captures the unique sub-clustered representations within each disease class, enabling better characterization of feature distributions. Specifically, SCAN follows a dual-branch framework, where the first branch learns class-wise features to distinguish different skin diseases, and the second branch aims to learn features which can effectively partition each class into several groups so as to preserve the sub-clustered structure within each class. To achieve the objective of the second branch, we present a cluster loss to learn image similarities via unsupervised clustering. To ensure that the samples in each sub-cluster are from the same class, we further design a purity loss to refine the unsupervised clustering results. We evaluate the proposed approach on two public datasets for few-shot skin disease classification. The experimental results validate that our framework outperforms the state-of-the-art methods by around 2% to 5% in terms of sensitivity, specificity, accuracy, and F1-score on the SD-198 and Derm7pt datasets.

==> figures/fig6.tex <==
\begin{figure*}
\centering
\includegraphics[width=.95\textwidth]{figures/fig6.pdf}%插入图片，[]中设置图片大小，{}中是图片文件名
%\captionsetup{labelfont={color=blue},font={color=blue}}
\caption{Impact of the proposed cluster branch on features in the base classes of SD-198 dataset. The t-SNE visualization results of 20 base classes are shown in a) without clustering branch and b) with clustering branch respectively.} %最终文档中希望显示的图片标题
\label{fig6} %用于文内引用的标签
\end{figure*}

==> tables/table6.tex <==
\begin{table}
    \centering
    \caption{The calculation of inter-class variance $D_{inter}$, intra-class variance $D_{intra}$ and discriminative function $\phi$ on the novel classes of SD-198 and Derm7pt datasets.}
    \begin{tabular}{c|c|ccc}
    \toprule
    Dataset&Method&$D_{inter}(C)$&$D_{intra}(C)$&$\phi(C)$\\
    \midrule
        \multirow{2}*{SD-198} & Baseline \cite{chen2019closer} & 0.265644 & 0.250569 & 1.060161 \\
        ~ & SCAN (ours) & 0.259522 & 0.226078 $\downarrow$ & 1.147933 $\uparrow$ \\
        \hline
        \multirow{2}*{Derm7pt} & Baseline \cite{chen2019closer} & 0.109657 & 0.365394 & 0.302087 \\
        ~ & SCAN (ours) & 0.103585 & 0.244574 $\downarrow$ & 0.424906 $\uparrow$\\

    \bottomrule
    \end{tabular}
    \vspace{-2mm}
    \label{table:phi_value}
\end{table}
